Benchmarking JSON BinPack

In this paper, we present benchmark results for a pre-production implementation of a novel serialization specification: JSON BinPack. JSON BinPack is a schema-driven and schema-less sequential binary serialization specification based on JSON Schema. It is rich in diverse encodings, and is developed to improve network performance and reduce the operational costs of Internet-based software systems. We present benchmark results for 27 JSON documents and for each plot, we show the schema-driven and schema-less serialization specifications that produce the smallest bit-strings. Through extensive plots and statistical comparisons, we show that JSON BinPack in schema-driven mode is as space-efficient or more space-efficient than every other serialization specification for the 27 documents under consideration. In comparison to JSON, JSON BinPack in schema-driven mode provides a median and average size reductions of 86.7% and 78.7%, respectively. We also show that the schema-less mode of the JSON BinPack binary serialization specification is as space-efficient or more space-efficient than every other schema-less serialization specification for the 27 documents under consideration. In comparison to JSON, JSON BinPack in schema-less mode provides a median and average size reductions of 30.6% and 30.5%, respectively. Unlike other considered schema-driven binary serialization specifications, JSON BinPack in schema-driven mode is space-efficient in comparison to best-case compressed JSON in terms of the median and average with size reductions of 76.1% and 66.8%, respectively. We have made our benchmark results available at jviotti/binary-json-size-benchmark on GitHub.

==> Makefile <==
include vendor/vendorpull/targets.mk

.DEFAULT_GOAL = all

assets/benchmark/%.png: scripts/plot.py vendor/binary-json-size-benchmark/output/%/data.dat \
	vendor/binary-json-size-benchmark/benchmark/%/NAME vendor/binary-json-size-benchmark/benchmark/%/TAXONOMY
	/opt/homebrew/anaconda3/bin/python3 $< $(word 2,$^) "$(shell cat $(word 3,$^))" "$(shell cat $(word 4,$^))" $@

all: benchmark.tex \
	$(foreach document,$(wildcard vendor/binary-json-size-benchmark/benchmark/*),assets/benchmark/$(notdir $(document).png))
	pdflatex -halt-on-error -file-line-error -output-directory=. $(basename $<)
.PHONY: all


==> sections/acknowledgments.tex <==
In no particular order, many thanks to Ben Hutton and Kris Zyp for helpful
discussions regarding JSON Schema and its history.

